A Study of Opacity Ranges for Transparent Overlays in 3D Landscapes

{When visualizing data in a realistically rendered 3D virtual environment, it is often important to represent not only the 3D scene but also overlaid information about additional, abstract data. These overlays must be usefully visible, i.e. be readable enough to convey the information they represent, but remain unobtrusive to avoid cluttering the view. We take a step toward establishing guidelines for designing such overlays by studying the relationship between three different patterns (filled, striped and dotted patterns), two pattern densities, the presence or not of a solid outline, two types of background (blank and with trees), and the opacity of the overlay. For each combination of factors, participants set the faintest and the strongest acceptable opacity values. Results from this first study suggest that i) ranges of acceptable opacities are around 20-70%, that ii) ranges can be extended by 5% by using an outline, and that iii) ranges shift based on features like pattern and density.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> chapters/02-related-work.tex <==



\section{Background}
\label{sec:Related_Work}

% I have largely redone the first subsection of the prior work, and hopefully this can be both a better survey for the graphics techniques and an example for the other subsections in prior work
% One important thing to remember is that the paper is a very concise report for a expert community, not for a general audience. So we never start with the baseline concepts as one would when writing a textbook. Instead, we assume that everyone reading this is already an expert with this field and only brush up the most relevant materials, and make a connection from these materials to our work. 
% This is different from a thesis. In your thesis you can start from square 1 and go all the way to square 10, and write a few pages on it. In a paper our starting point is usually already square 8 or 9, then only make the last critical step here. - lucky


%\RED{Maybe not the first subsection. Or maybe this will be a "interrim" paragraph in section 2 but without a subsection title}

%\subsection{Visualization and Real-time Photorealistic Rendering}
Our research is motivated by the recent adoption of real-time and high-performance photorealistic rendering in industrial data visualization applications, and in particular, high-fidelity GIS-based visualization applications~\cite{digitaltwin,cesiumstory,ESRIArcGIS}. 
These widely-used tools and their eco-systems form the backdrop of our research 
and provide initial design references for the configurations of overlays we investigate in this paper.

%Unlike games that use the realistic environment to drive narration and experience, productivity and analytical tools aim at presenting accurate information and providing precise analytical manipulations of the data~\cite{marriott2018immersive,riche2018data}. 
%Below, we discuss relevant prior work on graphical perception, the importance of opacity, and the graphics implementations of overlaid colors in 3D rendering.

%\charles{Here I would rather talk about how 3D is coming back to being hype, how immersive environments and VR are exploding, and how industrial applications are embracing this trend to visualize data in immersive environments. Perhaps give some well-known examples or typical scenario/case study like the one in the intro about the tree-cutting areas, perhaps even with some images.}

%\RED{I agree but these (industrial trends VR hype etc) does not have peer-reviewed citations and only has a ecological relevance to the research, but essentially is not part of the scientific inquiry here.
%\\
%I removed the subsection title, added some text and some reference, so it ends up more like an General Statement but not a serious part of the background survey}

%\charles{to me where this paragraph is going (what we used in the study) should be in the study section - we should not talk about the user study nor the specific implementation we used here}
%\RED{agreed, we'll move the next paragraph out of related works(keep the citations!)}
%\charles{yes, keep citations}
 

%

%moved from introduction
 
%How to drive efficient productivity and analytical tasks in a realistic 3D virtual environment is an open research problem, which cannot be solved by known methods from the entertainment applications~\cite{AVRNextGen}. 


%Highlighting in general has a very broad meaning and can be defined for various purposes. The definition of the Cambridge Dictionary is "to attract attention to or emphasize something important". But how or what do we try to emphasis? This is highly dependent on the context. 

%Through collaborating with an industrial partner specialized in 3D visualization in realistic environments, we identified the importance of visually conveying abstract data in these scenes.

%There are a few interactive tools for 3D environments which uses abstract data overlays. [...] These tools usually use the object itself to apply additional information visualisation on top. For example changing the color of an engine part in a training environment to highlight the currently important part. The main difference to our project is that for this kind of work the object itself is the part which needs to be emphasised. Thus the emphasised shape is already known in 3D coordinates and a simple shader can be applied to change the objects appearance. Within our project we try to create a abstract overlay in a digital 3D environment from a 2D data set, thus we don't know what exactly will be inside our area of interest. There might even be objects on the edge of this area. An additional challenge in our approach is that we don't want to highlight the whole mesh. For example we have some specific area we need to highlight on our terrain. Here we don't want to highlight the whole terrain but only certain parts of interest. Within the training environments state above these shape would be modeled within the world and shaded accordingly. Our approach is supposed to be more generic, so it can be applied to any kind of terrain without remodeling the environment every time the area of interest changes.


%\subsection{Graphical Perception Studies}
%============================================================================%
% Subsection presents graphical perception studies in general
% - graphical perception studies are useful to establish guidelines
% - mostly done in infovis
% - some are done in SciVis (e.g., DeadEye and DeadEye Revisited)
% - none were done about overlays. This requires design decisions and implementation decisions.
%============================================================================%

Creating an overlaid visualization that would sit on top of a photorealistic, 3D environment, such as the example shown in Figure~\ref{fig:teaser} requires a visualization designer to make choices. 
These choices are currently very limited, as they are inherited from 2D GIS tools and constrained to a transparent layer of color being displayed on top of the realistically rendered landscape~\cite{GeoVisBook}.
To think beyond this conventional design We can turn to the field of information visualization, that provides many empirical guidelines for representing abstract data, established through graphical perception studies~\cite{cleveland1984graphical}. 
Graphical Perception studies in information visualization, however, make strong assumptions regarding the background and environment in which the abstract data is being represented, typically a uniform background or a 2D map and a static point of view. In contrast, 3D landscapes are colorful, contain complex geometries and textures, and can be looked at from infinite numbers of points of view. It makes it difficult to directly apply results from studies that consider standard 2D charts (e.g.,~\cite{gutwin-emphasis,haase2000meteorology,hughes2001just,bartram-whisper}).
%For example, while we know that there are many ways to draw attention to -- or emphasize -- a particular area of interest in a visualization, for example by manipulating visual variables~\cite{bertin1983semiology}, we also know that emphasis effects which are created by being overlaid on the foreground of the rendered scene are influenced by the background of the scene~\cite{hall2016formalizing}.
%It is known that results from graphical perception studies depend even on the dataset being used~\cite{kim2018assessing},making it unlikely that guidelines from graphical perception studies based on standard 2D charts directly apply to 3D environments. 
%This observation has led to a recent increase in graphical perception studies in virtual reality environments (e.g.,~\cite{marriott2018immersive,bach2017hologram}) and to the investigation of preattentive features in scientific visualizations~\cite{krekhov2018deadeye,krekhov2019deadeye}.

%Despite this increasing body of work at the edge of several sub-areas, to the best of our knowledge there exists no empirical investigation to establish how people perceive overlays in photorealistic 3D environments. This is important not only to know how to highlight an area of interest, but also to communicate abstract data dimensions to the viewer by using visual variables~\cite{bertin1983semiology} to vary the appearance of the overlay.
%Earlier work showed for example that color is an important factor in the perception of categorical data sets. 
%Green et al. \cite{green1998toward} proposed an automation for, the selection of different color palettes based on the principles of human visual perception of categorical data and, to identify regions where visibility is hindered by a visually dominant structure. 
%Csinger et al. \cite{csinger1992psychology} proposed multiple physiological, perceptual and cognitive guidelines when using color as feature for encoding information. 
%Other psychophysical theories have shown that color, orientation, contrast, size and luminance are important factors for visualising textures, and it has been shown that certain configuration can be perceived faster than others~\cite{csinger1992psychology,gallostudy}. 



%\subsection{Focusing on Opacity}
%============================================================================%
% Presents our focus on transparency
% - In this paper we need to focus on one aspect to study. We look at transparency.
% - transparency is very good to convey quantitative information
% - transparency has been studied previously, and we take inspiration from a previous study~\cite{whisper}.
%============================================================================%
%The opacity of overlays is an important variable to investigate, because it is well-suited to landscape environments and can occlude other objects in the scene.

We already know that displaying tools for interactive environment in a semitransparent way can increase the selection and navigation capability compared to fully opaque tools~\cite{zhai1996partial}, and are helpful for guiding users in virtual environments \cite{schmalstieg1999using}. 
%To increase the visibility of windows, the unimportant part can be rendered in a transparent way to see the content below the window. 
This way, the amount of visible content can be increased~\cite{ishak2003free}. 
%Harrison et al.~\cite{harrison1996experimental,harrison1995experimental} investigated how transparent menus and interfaces affect the visibility of the content. They considered different configuration of backgrounds of text pages, wire-frame images, and solid images and showed that the background as well as the chosen transparency, have an strong impact on the readability of the content. 
Transparency/opacity is also an effective visual variable to encode quantitative information~\cite{munzner-book} such as uncertainty~\cite{collins2007visualization} of the RoI, and has been the focus of studies on the perception of grids in 2D charts~\cite{bartram-whisper}.
%and by adjusting or blurring the surrounding areas\cite{robinson2006highlighting}. 
%Transparency in visualization: See Section 3.3 in Whisper paper: \url{https://research.tableau.com/sites/default/files/2011-WhisperGrids.pdf}
The previous work showed that opacity is an important factor when viewing or interacting with layered levels of information. 
Most of this work has been conducted in 2D applications, and in this work we contribute to this line of research by extending it to 3D landscape environments.



%\subsection{Color Overlays in Visualization and Graphics}
%============================================================================%
% Subsection presents the context/background and shows it's an important problem to solve
% - it is a very important thing to have, and it is used already in commercial tools. Give examples of why it is important, and how it is used, as well as what they look like and how they are implemented
% - our partner told us it's important too - background from LlamaZOO's expertise/practice
% - there are many parameters/variables we could use, and a few are often made available (color of block and transparency?)
% - some research has looked at highlighting in 3D scenes
% - some research has looked at representing abstract data in 3D scenes
% - but we don't have guidelines for how to best design and implement these overlays
%============================================================================%
%\RED{I thought we have decided never mention the word ``highlight'' right?}
%\\
%\RED{Moved implementation background review to the last subsection.}



%Color overlays are commonly used to visually accentuate part of a 3D model in both computer graphics and industrial visualization applications (see Figure~\ref{fig:google_earth}). 
%Modelling tools routinely use an overlay of color to indicate the focused part of manipulation (Figure~\ref{fig:mayarig}); while the visualization community has employed varying surface colors to delineate properties of different parts on a surface~\cite{MedicalVisBook}. 
%The graphics implementation of color overlay can be straightforward, by changing the material property of a mesh or modifying pixel colors in a texture when surface parametrization is available. 

%In Direct Volume Rendering (DVR), visual surfaces are constructed in the rendering process from a discrete point set, and surface color overlay can be configured as part of the rendering~\cite{DVRLighting, MedicalVisBook}. 

%A common, yet slightly more difficult situation arises when the 3D model is explicit (mesh) but has no suitable surface parametrization for locating the overlaid color. 
%For example, a feature dataset may describe a spatial property of one part on a mesh using world-space coordinates, while the mesh surface is parametrized in a local UV coordinate system for texturing. 
%In this case, we cannot directly render the dataset by adjusting pixel colors on a texture, but there are a few known ways to handle this situation for raster graphics. For instance, the feature data can also be modelled as a mesh, and the coloring part can be computed via an \textit{intersection} operation using Constructive Solid Geometry (CSG) methods~\cite{CSG2016}. 
%The resultant mesh is a single explicit surface that equals to the part of the original model delineated by the dataset, and can be rendered in an additional pass on top of the original model. 
%The CSG intersection can be either implemented as a pre-processing step, or as part of the rendering runtime by using the image-space CSG methods~\cite{hable2007cst}. 

%Additionally, we can locate the overlaid color in the image space by first recording the world-space coordinate in the framebuffer for each pixel, then query the feature dataset in a post-processing sampling step to determine whether the pixel is inside or outside the feature. We implemented and evaluated a few graphics methods in our research as discussed in section~\ref{sec:implementation}.

==> chapters/06-implementation.tex <==
\section{Implementation}
\label{sec:implementation}

%To perform the user study we had to provide an implementation to be able to display the overlays in the given environment. While doing so we considered real world challenges to create an implementation which can solve those challenges and is able to visualize the given overlays. The biggest challenges were to be able to support large growing environments and their numerous amount of overlays. Thus, after careful consideration we choose three different techniques to implement and compare, one vectorized and two rasterized solutions, each with different approaches about quality, performance and scalability. 

Because we investigate visualization in an interactively rendered environment, the rendering implementations are impactful to the visualization experience. In this section, we discuss our graphics implementation of the overlaid visualization and compare their advantages.  
Our experiment platform is the Unity game framework with its Physically-Based Rendering (PBR) raster-based real-time graphic system~\cite{UnitySoftware,PBRBook}. 
PBR is an empirical shading method capable of creating realistic appearances of common real-world materials, and the method is more versatile and accurate compared to the classical shading methods, such as the Blinn-Phong reflection mode~\cite{PBRBook}. 
In turn, PBR delivers high fidelity and vivid renderings which typically make uses of the full color gamut and dynamic range of a display device, leading to our investigation of how to coalesce abstract visualization with a PBR visual context.

We used three graphics methods for rendering the overlaid colors on top of the digital landscape: 
(1) image space Solid Constructive Geometry (CSG), (2) a Unity feature called Decal Projector~\cite{UnityDecal} and (3) a post processing sampling (PPS) method. 
The rendering methods is important to the visualization design and evaluation because it affects the frame rate of the program and visual clarity  of the overlaid color in the 3D scene. Our source data for defining the RoI of the overlays is in GeoJSON~\cite{GeoJSON}. 
In an offline pre-processing step, we convert GeoJSON to either (1) a three-dimensional mesh that conform to the shape defined in GeoJSON and extruded to a large extend, for the CSG rendering method, or (2) a rasterized image from the shape defined in GeoJSON, for the Decal Projector and PPS methods. 
Below, we briefly introduce these three graphics methods, compare them based on their rendering performance and scope of application, and evaluate their usability.


%============================================================================%
% Section describes all implementations and their comparison
% - there are several ways of implementing overlays
% - we identified these 3 (why? are there others?)
% - we compared them (along 2 dimensions: performance and coverage of designs)
% - secondary contribution: table that compares what designs each implementation supports. based on this comparison we selected X for our study
%============================================================================%

%\subsection{Preprocessing}
%To prepare the data for the rendering we have to perform additional preprocessing of the incoming data set. Here we use geo-spacial GIS data, which has to be transferred from a geographic coordinate space, consisting of latitude and longitude,  into a texture space and later into the world space of our digital environment. The input data consists out of several points in the geographic coordinate space, which are a representation of  2D shapes. For simplification we don't include the earth's curvature into this transformation. After the data has been transformed into the texture coordinates, we have to draw each shape to a texture, either one big texture or one texture for each shape. Here we can apply all design choices we want to make the overlaid area as desired, like choose different transparency values or changing the pattern style. For the CSG solution we use have to create a mesh instead of a texture.  





\subsection{Image Space CSG}

\begin{figure}[t]
   \centering
   \includegraphics[width=0.9\linewidth]{pictures/imcsg.PNG}
   \caption{A recreation of the surface color overlay example from Hable et al.~\protect\cite{hable2007cst} in Unity with image-space CSG. The part of the bunny intersecting the `CSG' shaped mesh becomes a yellow overlay.}
    \label{fig:csg}
\end{figure}

We use a simplified image space constructive solid geometry (CSG) method to create the overlaid colors on top of a 3D terrain model. 
In the pre-processing step, we create a shape mesh by extruding the 2D shape defined in a GeoJSON file in the dimension orthogonal to the planar shape.
We then place this extruded mesh with the terrain model and align the terrain's surface with the middle part of the extruded mesh. 
This way, we can consider the intersected part of the model mesh inside the shape mesh as the colored area that conforms to the GeoJSON definition. This area can be found by performing a \textit{parity count} for the fragments from the model against the shape mesh. 
Figure~\ref{fig:csg} illustrates this operation with an example recreated from Hable et al.\cite{hable2007cst}.     
%CSG has different use cases and is not limited to create overlays. The original use in video games was to create solid geometry models as boolean combinations of primitives. In our case we use a screen space solution of the CSG. To define the RoI we have to create a solid mesh from the given 2D RoI during the pre- processing step, also called the CSG volume. This mesh is the then used to create the overlay. Everything intersecting the mesh will be stored in a stencil buffer. With this stencil buffer we are able to identify where the overlay should be drawn. The approach of creating the stencil buffer can be separated into three phases: The first phase consist of a depth test between the CSG volume and the objects which the overlay should be applied to. For every pixel we check if the front faces of the CSG volume are in front the object. If this is true the stencil buffer value for this pixel will be increased for every front face before the object, as seen in Figure \ref{fig:csg}. During the second phase a similar depth test is performed, but this time the back faces of the CSG volume are considered. If those are in front of the of the object, the stencil buffer value will be decreased. Thus if the same amount of front and back faces of the volume are in front of the object the object is not inside the volume but behind it or in between a concave area of the object, the stencil buffer for this case would be 0. During the third phase every pixel with a stencil value of 1 will be blended between the original color value and the overlay's.

%the following is good but should be in the comparative analysis.
%Since this approach is vectorized the quality of the overlay does not change. No matter how close the view is to the overlay a high quality representation will be contained. Creating outlines using CSG reacquires to render the overlay twice, once for the interior and once for the outline itself.

\subsection{Decal Projector}
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{pictures/decal_sketch.png}
%    \caption{Pipeline of creating the Decal Mesh }
%    \label{fig:decal}
%\end{figure}
Unity's Decal Projector is an open source feature that renders a texture overlay on any part of a 3D scene without requiring a consistent paramterization or UV map across the scene~\cite{UnityDecal}. 
It only requires a texture image, and parameters of a ``projector'' such as location, direction and Field-of-View (FoV).
The texture image is overlaid on top of the rendered scene like a slide projector would project an image on a wall.

Unity implements this feature by back-projecting pixels in the frame buffer to an additional camera space defined by the projector parameters with linear perspective, and shade the pixels according to their coordinate on the image plane of the additional camera space, where the user texture can be sampled. 
In our experiment, we supply the Decal Projector with the texture we created from the GeoJSON file in processing and project it onto the terrain. We use the decal projector as a tool and do not modify the Unity implementation. 
We build visualization features such as outline and various patterns into the projected texture in the pre-processing step. 

%With this techniques no UVs for the projected surfaced are needed, they will be created based on the given vertex coordinates in the projection range. The projection range is usually defined by a box shape and a projection direction. Every object inside the box will have the texture projected from the given projection direction. To internally create UVs the objects have to be cropped to the projection range. We take every model within the box, transform it into the projector space and cut away everything that is not in the projector box. Since the projector box is a rectangular shape we can derive UVs based on the vertex position inside this box. This way we create our cropped decal mesh with UVs, which we now transfer back into the world space and assign the given texture to it. Additionally the position and size of the decal projector have to be determine during the preprocessing step, and afterwards be applied to the scene to position every overlay at the correct location. Decal projectors support various sizes of projection texture based on the quality required. Which level of quality is feasible depends on the application. If the overlays are further away a lower quality texture will be sufficient. Adding outlines for Decal Projectors can either be very expensive or remove the ability to change the pattern independent from the outline during runtime. Since the projected texture is considered as a single texture, we either have to draw the outline and the internal pattern into one texture during the pre-processing step, which makes them dependent on each other, or we separate the outline and the internal pattern into two separate textures and draw them on top of each other, which doubles the amount of projectors necessary, but gives us the possibility to exchange pattern and outline during runtime.

\subsection{Post Processing Sampling}
The third implementation we tried is similar to the decal projector but with a simplified image-space post-processing sampling (PPS) strategy.

In this implementation, we first record the world-space coordinate for each pixel in an additional frame buffer during the 3D rendering. 
Then, we use the recorded world-space coordinate to sample into the texture created from the GeoJSON file with an additional image-space post-processing pass. 
The sampling coordinate can be calculated following the mapping between the world-space coordinate system in Unity and the GIS coordinate system in GeoJSON. 
This implementation does not need the back-projection step in Unity's Decal Projector, but requires to manually set up the coordinate transformation between Unity's world-space and GeoJSON's coordinate systems.   

%This approach combines a image space post processing effect with an additional world position render layer. During the pre-processing step, a lookup texture is created which can later be used to define which area lies within an overlay. This lookup texture corresponds to the size of the environment, each pixel in the texture represents a specific area within the environment; the larger the texture, the smaller the corresponding area, the higher the quality of the overlays. Therefore the size of the environment must be known during the pre-processing step. To be able to distinguish between overlays and to enable or disable certain overlays at runtime, we encode IDs within the given texture layers (RGBA). At this point we reserve one byte to encode the outline position in order to be able to crosscheck them individually. This lookup texture is later used to determine if the pixels on the screen are within a RoI and if the given pixel belongs to an outline. To crosscheck these values for each pixel, the corresponding world position of every object the overlay should apply to is required. Thus, we create a rendering layer containing those objects. Each individual object within this layer has its world position drawn to an off-screen render texture based on the perspective of the camera. This only works for opaque objects, however, thus the world position of each pixel is known. In the post-processing step, these world positions are compared with the previously created look-up texture. If the corresponding pixel in the lookup texture has a value greater than 0, this pixel belongs to a RoI and it has to be render based on the chosen visualization. So far, we have only determined if a pixel belongs to a RoI, but not how these areas should be rendered. To determine which pattern to use, the desired visualization style has to be transformed into a texture loaded into the shader. Here no UVs are needed, the texture can be sample according to the world position. For the post processing step the pixel's color values is already know. To add the visualisation to the current value we interpolate between both, the on screen pixel value an the sampled visualisation's color value weighted by the desired opacity. This way we these visualizations can be adapted during runtime. To enable the border, we have to check if the corresponding ID of the reserved border byte in the lookup texture is set to 1. For each pixel where this is the case, the color value of the border is determined similar to the patterns, by interpolating. 



%Thereby we have to reserve on byte to encode the outline position in order to be able to crosscheck it individually. This texture is later used to determine if the pixels on the screen are within a RoI and if the given pixel belongs to an outline. The be able to cross reference those value for every pixel on screen we require the world position of every object we want to apply the overlay on. Thus we create a rendering layer and all objects that should be included into this layer. Every single object within this layer has its world position drawn to an off-screen render texture based on the camera's perspective. This only works for opaque objects. However, thus we know the world position of every relevant object. During the post processing step we cross reference those world positions for every pixel to the prior created look up texture. If the given pixel in the lookup texture has a value greater 0 we know this pixel belongs an RoI and we have to render it based on the chooses visualisation. So far we have only determined if a pixel belongs to an RoI, but not how to render those areas. To determine which pattern to use we have to load the desired visualisation style as texture into our shader and sample them according to their world position and interpolate the texture's color value with the pixel's color value weighted by the chosen opacity value. Thus we can adapt those visualisations during runtime. If we want to add the border we only have to check if of the given ID of the reserved border byte in the lookup texture is set to 1. For every pixel where this is the case we add the border's color value as we do for the pattern's. 
 %Thus we create a emit World Position layer and add all necessary objects. Every object within this layer will render its world position position into an offscreen render texture. Thus we store the world space coordinates for every on screen pixel. Note that this only works with opaque objects, since we can only have one value for each pixel.




%As last and final step we apply our choice of design to the highlight area as post-processing effect. Thus the performance it not bound to the amount of highlights we use, but rather to the size of our environment and the displayed resolution\todo{is this true?}. Within the post-processing shader we check for every pixel on our screen if the corresponding xyz world space coordinate is within a highlight area by looking up the XZ world coordinates in our, in the first step created, look up data structure. This way we can also check to which highlight this pixel belongs and handle them according to our design of choice.

\subsection{Comparative Discussion}
\begin{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{pictures/DrawCalls.png}
    \caption{Amount of draw calls for increasing amount of overlays }
    \label{fig:drawcalls}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{pictures/SetPassCalls.png}
    \caption{Amount of set pass calls for increasing amount of overlays}
    \label{fig:setpass}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{pictures/Vertices.png}
    \caption{Amount of vertices for increasing amount of overlays}
    \label{fig:vertices}
\end{figure}

\end{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{pictures/RenderTime.pdf}
    \caption{Render time per frame plotted against number of overlays.}
    \label{fig:rendertime}
\end{figure}

We now compare the rendering performance, visual quality and tool usability of the three graphics implementations, and discuss their advantages and disadvantages.

To measure rendering performance, we successively added layers of overlays to our scene and measured per-frame render time (Figure \ref{fig:rendertime}). 
We used a laptop with an Intel i7-9750 CPU, 32GB RAM and a Nvidia Quadro T2000 graphics card with 4GB GRAM for this experiment. 
We found that the decal projector is most impacted by the amount of color layers added, followed by the image space CSG method. 
The PPS method show a near-constant performance impact. 
By profiling the program, we observed that the decal projector is the most expensive rendering operation among the three for additional color shapes and RoIs, while a simple texture sampling in the PPS method incurs negligible rendering cost. 
Therefore, for visualization tasks with a heavy data load, we recommend the PPS method, while the other two methods can be also used when the size of data is small.

Secondly, we compared the visual quality of the rendered color overlays. 
both decal projector and PPS are rasterized methods that rely on texture sampling. Thus, they show aliasing when rendered from a point of view that is close to the surface of the terrain model.
On the other hand, the CSG method uses a mesh to define a region of the surface that needs to be colored, and delivers a vectorized, resolution-independent rendering of the boundaries of the color overlay. 
Therefore, we recommend to use image-space CSG for surface overlay renderings that must be rendered at a  close distance to avoid the aliasing artefacts caused by texture sampling.

Lastly, we qualitatively comment on the usability of the three implementations for a visualization developer. 
Being a production feature in the Unity game framework, the decal projector is the easiest to use, with well-defined user interfaces and live preview functionalities built in Unity. Both the image space CSG method and the PPS method require a visualization developer to write customized rendering programs, which requires a 3D rendering background.

The CSG method renders the color overlay by modelling a new shape mesh and intersecting the shape mesh with existing models. 
To our experience, this mesh creation and placement operation can be familiar to content artists who routinely work on 3D scene creation. 
On the other hand, the PPS method requires one to derive a coordinate transformation between the 3D scene's world space and GeoJSON's coordinate system. This task requires the developer to understand the involved mathematics, cannot be interactively previewed, and can be error prone if multiple GeoJSON files with different coordinate systems are used in one visualization.
Therefore, we recommend using the decal projector for visualization designers with limited programming background, while the CSG and PPS approaches are more suitable for professional development teams experienced in graphics programming and 3D content creation.     

%All of these measurements showed that for the PPS, after the initial drop in performance for enabling the technique, performance remained stable at a constant value. The CSG implementation showed almost constant growth in all measurements. The Decal solution showed almost constant growth in draw calls and set-pass calls, with a lower growth rate than CSG. The number of vertices changed almost unnoticed with additional overlays for DP. However, the time per frame seems to grow exponentially.

%The DP are already included in Unity's high definition render pipeline and thus provide an easy entry point to overlay visualisation. They are able to create high quality overlays as long as the number of overlays is small. For an increasing number of overlays more powerful systems are required to still ensure a real time experience. The quality of the overlays is exchangeable and allows to adjust the performance needs a little. Since DP is a rasterized solution the quality of textures has to be increase, once the view is getting close to the RoI, to remain a high quality overly. However, compared to CSG and PPS the cost per additional overlay is very expensive and seems to be exponential, thus we can only recommend DP for a small numbers of overlays. To avoid the need of exchanging texture for a higher quality we recommend CSG. Since this solution is vectorized it allows to zoom in to an infinite level and still remain a high quality result. Increasing the amount of overlays or the complexity of overlays (increasing the amount of vertices needed to describe a overlay) increases the performance needed in a linear matter. Both solutions, DP and CSG, increase the required performance when an outline is displayed. Both solutions must be run twice to enable outlines during runtime. While DP offers the opportunity  of adding cheap outlines when neglecting the possibility of treating them separately, CSG does not have this possibility. However, CSG is suitable for applications of any size and can handle a large number of overlays. The lack of cheap outlines can be compensated for by the infinite resolution when zooming and can therefore be useful for applications where the view is close to the overlays. PPS has a very unique performance feature, once the post processing layer is enabled in every frame every pixel will be cross referenced to the look up texture and decide if the given pixel is within a overlay or not. After this initial cost is does not matter how many overlays will be displayed the performance needed stays constant. This allows to display large numbers of overlays. Since the interior pattern is not influenced by the look up texture the pattern and outline can be adjusted easily during runtime. However, the biggest drawback of PPS is it's dependency on the size of the environment. Since the lookup texture represents the whole environment, the area a pixel decodes increases if the environment increases. Thus the quality of the overlays depends on the environment size, and for high quality results PPS is only feasible in medium to small environment. However within this environments PPS is a good solution when rendering large numbers of overlays, since compared to CSG and DP the render time per frame is not dependent on the amount of overlays. This solution can also grow with the ability of loading huge data structures to the GPU. 


\begin{comment}

DP pro: easy to use and fast to setup to create some tests. Allows high and low quality settings which can be changed based on needs
Dp con: compared to other techniques expensive, especially when increasing the amount of overlays. Borders are either expensive or limit the runtime usability 
Dp Usecase: For a quick setup in scene with low amount of overlays suitable, can even create high quality results, independent of size of the environment .

CSG Pro: verctorized results, infinite resolution, infinite zoom in 
CSG Con: increased number of overlays or more complex overlays (vertices are important) create more complex meshes which leads to increased computational needs. Outlines are expensive, doubling the amount of overlays created. No cheap way to create outlines  
CSG UseCase: Since the very high infinite resolution good for application were the view is very close to the edge of the overlay. Independent of environment size. can handle medium to high amount of overlays 

PPS pro: very fast after initial cost, no additional render time for adding overlays, no additional cost for borders based on ID in texture, supports large numbers of overlays, easy to exchange pattern or turn outline on or off
PPS con: Quality is dependent on the environment size. Ever pixel in lookup texture represents a certain area in the environment, a larger area leads to increase the area one pixel in the texture represent in the environment, if not zoomed in to close also usful for large environments 
PPSUseCase: Medium to small environments, with large numbers of highlights which can be changed during runtime 
\end{comment}



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

